Image-Hashing-Based Anomaly Detection for Privacy-Preserving Online Proctoring

Online proctoring has become a necessity in online teaching. Video-based crowd-sourced online proctoring solutions are being used, where an exam-taking student's video is monitored by third parties, leading to privacy concerns. In this paper, we propose a privacy-preserving online proctoring system. The proposed image-hashing-based system can detect the student's excessive face and body movement (i.e., anomalies) that is resulted when the student tries to cheat in the exam. The detection can be done even if the student's face is blurred or masked in video frames. Experiment with an in-house dataset shows the usability of the proposed system.

==> sections/experiment.tex <==
\section{Experiments}
\label{Sec:Experiment}

\subsubsection{Data Collection and Analysis}
\paragraph{Self-made Anomaly Videos}
The dataset that is required for this project is too specific and there are no publicly recorded videos of students taking exams, so we created the needed videos by ourselves. Each team member recorded approximately one-minute video following the instruction (Appendix \ref{Appendix_instruction}) using common computers with a web camera. Both normal behaviors and anomaly behaviors are recorded and after each action, it is required to look at the center of the screen for two seconds. Normal behaviors include looking at the center, looking at the keyboard, etc. While, abnormal behaviors include looking sideways, getting up, and so on. After the video is finished, the labels indicating when the action is done are tagged by ourselves for testing the ability of the anomaly detection model. These self-made anomaly videos are used to select detectors and to decide the blur level since no suitable video dataset is in public.

With the basic function of OpenCV (useful package in computer vision), the basic information of each video could be obtained (\ref{tab:5_table_2}).

    \begin{table}[h]
    \centering
    \begin{tabular}{lllll}
    \toprule
    Video Name & Size & Resolution & Duration & FPS  \\ \midrule
    Doris\_anomaly.mp4 (v1) & 87.2MB & 1280x720 & 1''05' & 30\\
    Jason\_anomaly.mp4 (v2) & 19.1MB & 1280x720 & 1''32' & 25\\
    Vivi\_anomaly.mp4 (v3) & 43.2MB & 1080x720 & 52' & 26.17\\
    Yang\_anomaly.mp4 (v4) & 26.4MB & 1280x720 & 1''14' & 30\\
    Mill\_anomaly.mp4 (v5) & 75.2MB & 1280x720 & 58' & 29.54\\
    \bottomrule
    \end{tabular}
    \caption{The basic information of self-made anomaly videos.}
    \label{tab:5_table_2}
    \end{table}


\paragraph{Public Datasets}
\label{modulemethod}
Because our self-made anomaly videos are limited (only five videos and all of the team members are Asian aged between 24 to 27), the evaluation result and the decision made based on these videos are not convincing enough. Therefore, some public datasets collected from GitHub or Kaggle are used to verify the result made by self-made anomaly videos and to check leaks. When analyzing public datasets, the main technique is OpenCV as well. 

\subparagraph{Model Selection}
The comparison between face detection models and eye detection models used the UTKFace dataset, CelebFaces Attributes dataset (CelebA), and HELEN dataset because these datasets provide the true position of facial landmarks, and then it is possible to evaluate the accuracy of detectors.

\textbf{UTKFace (aligned$\_$cropped) Dataset \citep{UTKFace}:} The UTKFace dataset is a large-scale face dataset with a long age span (range from 0 to 116 years old). The dataset consists of over 20,000 face images with annotations of age, gender, and ethnicity. The images cover large variations in pose, facial expression, illumination, occlusion, resolution, etc. There are two zip files from the data page: ``In-the-wild Faces'' and ``Aligned $\&$ Cropped Faces'' (with a text file containing the position of 68 facial landmarks). The images in the ``In-the-wild Faces'' file have some background information and body information, with a resolution of 200x200. Whilst, in the ``Aligned $\&$ Cropped Faces'' file, only a big face is in one image. When doing the detector selection, the ``Aligned $\&$ Cropped Faces'' file is used since it has the corresponding facial landmarks information.

\textbf{CelebA Dataset \citep{CelebA}:} This dataset is a popular computer vision and deep learning dataset. It is large as well with more than 200K celebrity images, with 10,177 unique identities, 40 binary attribute annotations per image, and 5 facial landmark locations. The images in this dataset cover different facial expressions, large pose variations, background clutter, and the resolution of images in this dataset various.

When experimenting, the first 2,000 images in this dataset are selected.  Since the resolution of images is various, the image resolution distribution plot (Appendix \ref{Appendix_celeba}) is created by OpenCV. From that plot, it is known that the resolution of most chosen images is 800x800. 

\textbf{HELEN Dataset \citep{HELEN}:} Helen dataset is quite small, consisting of only 2,330 high-resolution images (2,000 training and 330 testings) with highly accurate, detailed, and consistent annotations of the primary facial components. The annotated facial images are gathered from Flickr, exhibiting a large variety in appearance (e.g. pose, expression, ethnicity, age, and gender) as well as general imaging and environmental conditions.

 The first 1,500 images of the HELEN dataset in the training set are selected for testing. From the resolution distribution plot (Appendix \ref{Appendix_celeba}), most of the chosen pictures have 1,000x1,000 resolution.

\subparagraph{Face Anonymizers Verification}
\label{datacollection}
As for evaluating the effect of privacy-preserving methods, four public datasets are tested, including the UTKFace (In-the-wild Faces) dataset, Real and Fake Face Detection dataset (RF), Celebahq dataset, and LFW dataset. The resolution of images influences the effect of blurring. If the image has low resolution, the effect of blurring will be weakened and the blur level should be increased to achieve the same privacy protection effect. So, more attention is paid to the resolution of images. In order to be close to the online examination situation, datasets with high-resolution images are focused. 

\textbf{UTKFace (In-the-wild Faces) Dataset \citep{UTKFace}:} As mentioned before, there is some background information and body information in the images in the ``In-the-wild Faces'' file, which is similar to the recorded video during the exam. However, the resolution of images in the ``In-the-wild Faces'' file is various and much lower than that of images in the ``Aligned $\&$ Cropped Faces'' file.

Since the resolution of most images in this dataset is quite low, there are 1,495 images with resolutions higher than 800x700 are filtered for experiments using OpenCV. The image distribution plot can be seen in Appendix \ref{Appendix_celeba}. 

\textbf{Real and Fake Face Detection Dataset (RF) \citep{RF}:} This dataset is created to train models that could recognize fake faces. It contains expert-generated high-quality photoshopped aligned and cropped face images in two folders: ``traning$\_$real" (1,081 images) and ``training$\_$fake" (960 images). The resolution of photos is 600x600, which is high enough for the big face images. When doing the evaluation, only the images in the ``traning$\_$real" folder are applied since our project is focused on real faces.

\textbf{Celebahq Dataset \citep{CelebA}:} The Celebahq dataset, which is the high-quality version of the Celeba dataset, consisting of 30,000 images in 1024x1024 resolution. 2,000 images are randomly selected for testing.

\textbf{LFW Dataset \citep{LFW}:} The LFW dataset is a famous face recognition dataset, consisting of more than 13,000 images of faces collected from the web. Each face in the dataset has been labeled with the name of the person pictured. The pictures are not cropped, with some background information and body information such as shoulders. The resolution of images in this dataset is low, only 250x250. There are 2,017 images in this dataset used for experiments in this project.

\subsection{Privacy Preserving}

\subsubsection{Detector Selection and Optimization}
\label{EE_PP}

\paragraph{Detector Selection}
As mentioned before, because of the limited data and maturity of the face and eyes detection model, the existing trained detector will be implemented in our project. According to researching results, the detection models in OpenCV, Dlib, MTCNN, and MediaPipe packages are widely used, have stable performance, and do not require high-performance computers when implementing. Therefore, it is decided to evaluate detectors in these packages using our self-made anomaly videos to select the most suitable model for our project. All experiments in the detector selection part are run on a local computer (i7-10710U, 16G RAM, Windows 10). The selection is divided into two parts: face detection and eyes detection. 

In terms of \textbf{face detector selection}, there are three steps.
\begin{itemize}
\itemsep0em
  \item \textbf{Step 1}: Split videos into frames and add ``face" or ``no face" label on each frame
  
  This is the preprocessing step. Processing a video is much difficult than dealing with images and the video is made up of pictures. Because of this, the videos are split into frames and these images are crucial in our project. Since the dataset used in this section is self-made, there is no label for each frame. In this situation, it is hard to evaluate the performance of detectors. Therefore, the labels should be added by ourselves and are recorded in an excel file. Label 0 indicates no face and label 1 means having a face in the image. The standard of having a face is decided by a paper which discovers that the presence of the eyes and the mouth in the image is highly correlated with its faceness score \citep{lr-22}.
  
  \item \textbf{Step 2}: Apply models on self-made videos and calculate detected rate
  
  Firstly, the file containing the label information of each video is read into Python. Then all tested models are applied on five anomaly videos and the detected rate for each is calculated. The definition of the metric is:

$$Detected\ rate = \frac{Number\ of\ faces\ detected}{Number\ of\ frames} * 100 \% $$
% detected rate = (number of faces detected)/(number of frames)×100$\%$.

  \item \textbf{Step 3}: Compare and evaluate
  
  The summary result for models in Dlib, MTCNN, and MediaPipe packages is shown in \ref{tab:performance_face} and the detailed result with other evaluated models could be found in Appendix \ref{modelcompare-face}.
\end{itemize}

    \begin{table}[h]
    \centering
    \begin{tabular}{llll}
    \toprule
    Model & FPS & Detected Rate\\ \midrule
    \textbf{Dlib} & 7.01 & 92.93\%\\ 
    \textbf{MTCNN} & 1.57 & 80.10\%\\ 
    \textbf{MeidaPipe (Holitstic)} & 21.85 & 91.44\%\\ 
    \bottomrule
    \end{tabular}
    \caption{The performance of different face detectors.}
    \label{tab:performance_face}
    \end{table}

It is clear that the face detector in the Dlib has the highest detected rate, whereas the speed of the detection process is quite slow. The MTCNN model is good at face recognition task \citep{lr-12}, however, it may not be proper for our task, with a lower detected rate and small FPS. The MediaPipe is the balanced performer, with a decent detected rate and could detect face fast. Besides, the detected rate of the MediaPipe model is a bit lower because the model could detect half face and according to the definition of the ``face" label in step 1, the half face is labeled as ``no face" label. Therefore, it seems that the MediaPipe model is the most proper face detector for our project.
~\\

When it comes to \textbf{eye detector selection}, the procedure is similar to that of face detector selection, whereas the method to calculate the detected rate is different.

\begin{itemize}
\itemsep0em
  \item \textbf{Step 1}: Apply models on self-made videos and calculate detected rate
  
  Without splitting videos into frames and adding labels in advance, the eyes detection models are applied on anomaly videos first, and then label ``not detected -0 "/``detected -1" is manually added frame by frame. Determining whether the eye detection is successful or not by checking manually is really time-consuming and subjective.
  
  The definition of ``detected" and ``not detected" should be determined carefully since the correct position coordinates of facial landmarks in each frame are not provided. The situation could be labeled ``detected" is that the position of eyes is corrected pointed out. The samples of ``detected" and ``not detected" can be seen in \ref{fig:6_table_2}. As for the calculation of detected rate, it is determined by this formula $Detected\ rate = \frac{Number\ of\ frames\ with\ correct\ eyes\ detection}{Nnumber\ of\ frames\ labeled\ as\ ``face"}$ because ``no face" frames should be removed.

%detected rate =  (number of frames with correct eyes detection)/(number of frames labeled as "face")

    \begin{figure*}[h]
    \centering
    \includegraphics[width=1\textwidth]{Doris_pic/detected.pdf}
    \caption{The situations of ``detected" and ``not detected" when doing eye detector selection.}
    \label{fig:6_table_2}
    \end{figure*} 

  \item \textbf{Step 2}: Compare and evaluate
 
  In the same way, the summary result for models in Dlib, MTCNN and MediaPipe packages is shown in \ref{tab:performance_eye} and the detailed result with other evaluated models could be found in Appendix \ref{modelcompare-face}.

    \begin{table}[h]
    \centering
    \begin{tabular}{llll}
    \toprule
    Model & FPS & Detected Rate\\ \midrule
    \textbf{Dlib} & 6.14 & 92.93\%\\ 
    \textbf{MTCNN} & 1.57 & 80.10\%\\ 
    \textbf{MeidaPipe (Holitstic)} & 21.85 & 97.41\%\\ 
    \bottomrule
    \end{tabular}
    \caption{The performance of different eye detectors.}
    \label{tab:performance_eye}
    \end{table}
\end{itemize}

It could be noticed that the MediaPipe model is the most suitable detector for eyes with a 97.41$\%$ detected rate and the FPS is 21.85 (largest). The detected rate of eye detectors in both the Dlib and MTCNN packages is the same as that of face detectors. The reason for this is that these two detectors could detect facial landmarks on basis of detecting a face. However, for the MediaPipe model, detecting facial landmarks is not limited to detect a face. It could detect face and eyes separately, according to the body information in the frame.

Combing the comparison results of the face detection model and eye detection model, it could be concluded that the MediaPipe model is the most suitable model for our project and the detailed flowchart of taking the MediaPipe model as the main model could be found in Appendix \ref{mediapipe}. However, our final flowchart of the privacy-preserving part does not use the MediaPipe model solely since the limitations of the MediaPipe model are discovered when it is applied to public datasets (details of this are described in Section \ref{verificationofdetector}).

There are some limitations of this experiment. Because the videos utilized in this experiment are made by ourselves, there are no truth labels (``face" / ``no face") and the correct position of eyes. The definition of different labels and the decision to make whether the image meets the definition are all decided by ourselves, which are subjective and not serious. The detected rate calculated here could only explain that there is something detected but the accuracy of the detection (whether the detected thing is face or eyes) is not illustrated. Also, the data used here is limited, only five one-minute videos, and the person in the videos are all team members (similar age, Asian). Hence, three public datasets mentioned in the Section \ref{modulemethod} are used to verify the comparison results in the next section.


\paragraph{Results Verification}
\label{verificationofdetector}
As mentioned before, the results made by self-made datasets should be verified using public datasets. In this part, UTKFace (aligned$\_$cropped) dataset, CelebA dataset and HELEN dataset are utilized. The detailed information and analysis of these datasets could be discovered in Section \ref{datacollection}.

With the correct locations of facial landmarks, both the detected rate and the accuracy of detection could be measured. Since the facial landmarks of different models are different, it is impossible to directly compare the coordinates of the face and eyes. For our project, we draw the bounding box of the face and eyes according to the top, bottom, leftmost and rightmost detected points around the face and eyes. The FPS, detected rate and average normalized error are metrics to evaluate detectors. The detected rate is defined same as that in the previous section: $\frac{Number\ of\ images\ detected}{Total\ number\ of\ images} * 100\%$. The higher the detected rate, the better. However, the detected rate could not explain the accuracy of the model. The accuracy is evaluated by comparing the truth and detected locations of facial landmarks and the average normalized error \citep{lr-28} is used here. First, denote the detected and truth landmark locations for landmark i as $d_i=\{d_{x,i},d_{y,i}\}$
 and $g_i=\{g_{x,i},g_{y,i}\}$, the $g_{le}$ and $g_{re}$ are the left and right pupil centers. The average normalized errors are then calculated as: $\frac 1 N\sum_i^N\frac{||d_i-g_i||_2}{||g_{le}-g_{re}||_2}$. The less average normalized error, the better. The summary result for the face detectors is shown in \ref{tab:6_table_4} and the summary result for the eye detectors could be found in \ref{tab:6_table_5}. In the summary result, only the results of the Dlib model and MediaPipe model applied on the HELEN dataset are shown since the resolution of images in the HELEN dataset is closest to that of videos that would be recorded during the exam. The experiment result using other public datasets could be found in Appendix \ref{dectector_pub}.



    \begin{table}[h]
    \centering
    \begin{tabular}{llll}
    \toprule
     & Dlib & MediaPipe & MediaPipe + Dilb\\ \midrule
    \textbf{FPS} & 2.71 & 11.21 & 5.40\\ 
    \textbf{Detected Rate} & 96.93\% & 78.67\% & 99.27\%\\ 
    \textbf{Average Normalized Error} & 2.65 & 4.30 & 3.99\\ 
    \bottomrule
    \end{tabular}
    \caption{The performance of different face detectors on HELEN dataset.}
    \label{tab:6_table_4}
    \end{table}

    \begin{table}[h]
    \centering
    \begin{tabular}{llll}
    \toprule
     & Dlib & MediaPipe & MediaPipe + Dilb\\ \midrule
    \textbf{FPS} & 2.62 & 9.86 & 6.08\\ 
    \textbf{Detected Rate} & 96.93\% & 78.67\% & 99.27\%\\ 
    \textbf{Average Normalized Error} & 0.72 & 4.27 & 3.55\\ 
    \bottomrule
    \end{tabular}
    \caption{The performance of different eye detectors on HELEN dataset.}
    \label{tab:6_table_5}
    \end{table}

According to the results in \ref{tab:6_table_4} and \ref{tab:6_table_5}, it is interesting to notice that the performance of the MediaPipe model is not good as that on our self-made anomaly videos, with a lower detected rate and higher average normalized error. This may be because that the MediaPipe has some limitations for the dataset with various poses, expressions, ethnicity, and age. However, considering its fast speed, it is still selected as the main model in the privacy-preserving schema. In order to make up for the deficiency of the MediaPipe, the Dlib model which performs excellently on the public dataset as well (with the highest detected rate and lowest error) is added into the privacy-preserving schema. The performance of the combined model is decent, with nearly 100$\%$ detected rate and the decreased error, at the cost of speed. Therefore, the combined model is in our final privacy-preserving schema and the details could be found in Section \ref{moduleoverall}.


\subsubsection{Blur Level Determination}
\label{blur}

As for the ``blur without eyes" method, the blur level is the main factor that could influence the effect of privacy-preserving. Generally, the higher the blur level, the better the effect. However, with a large blur level, the speed of blurring decreases a lot. So, a suitable blur level should be decided. The face identification model - FaceNet used in the ID verification part is implemented to evaluate the effect of privacy-preserving. The details of how to implement face identification using the FaceNet model could be found in Section \ref{ID}. The purpose of privacy-preserving methods is to ensure that the facial information displayed is not enough to identify a person and a proper blur level makes it impossible for the face identification model to recognize a person. The recognition rate is used as metric here, which is calculated as: $\frac{Number\ of\ faces\ recognized}{Number\ of\ faces\ detected} * 100\%$. The lower the recognition rate, the better effect of the privacy-preserving method. Since there is no recommended threshold of recognition rate in papers that indicates the success of privacy protection, according to our experiment and feelings, the threshold of recognition rate is set as 5$\%$ by ourselves. If the recognition rate is lower than 5$\%$, it could say that the privacy protection is successful. The faces that could still be recognized when the recognition rate is lower than 5$\%$ are shown in \ref{fig:6_new}. It could be seen that the recognized faces are those with a strong reflection in glasses or very blurring. In our opinion, it is really hard for a human to identify a person in that situation. Therefore, 5$\%$ is a suitable threshold of recognition rate.

    \begin{figure*}[h]
    \centering
    \includegraphics[width=1\textwidth]{Doris_pic/recognized.pdf}
    \caption{Recognized faces when the recognition rate lower than 5$\%$.}
    \label{fig:6_new}
    \end{figure*} 


The blur level is determined using our self-made anomaly videos and then is verified by public datasets. When conducting experiments, the threshold of cosine similarity is set as 0.5 not only because it is commonly used, but also because when the threshold of cosine similarity is 0.5, the probability of correct discrimination is 90$\%$ (according to the conclusion of experiment in Section \ref{cos-sim}). The first original frame of the anomaly videos is set as the reference to comparing with the blurred frames. The result is shown in \ref{tab:6_table_6}.

    \begin{table}[h]
    \centering
    \begin{tabular}{llllll}
    \toprule
    Blue Level & v1 & v2 & v3 & v4 & v5 \\ \midrule
    15 & 61.20\% & 46.71\% & 0.68\% & 5.35\% & 91.18\%\\
    20 & 14.64\% & 0.77\% & 0\% & 3.09\% & 39.51\%\\ 
    25 & 2.72\% & 0.63\% & 0\% & 2.19\% & 10.95\%\\
    30 & 0.81\% & 0.63\% & 0\% & 2.12\% & 3.37\%\\
    35 & 0.86\% & 0.79\% & 0\% & 1.25\% & 1.44\%\\
    40 & 0.69\% & 0.48\% & 0\% & 1.41\% & 0.36\%\\
    \bottomrule
    \end{tabular}
    \caption{The recognition rate of anomaly videos with different blur level.}
    \label{tab:6_table_6}
    \end{table}

It is discovered that with the increase of blur level, the recognition rate decreases. When the blur level is 30, for all videos the recognition rate is lower than 5$\%$ and then it could be concluded that the suitable blur level is 30 for our anomaly videos. In order to confirm that this blur level is suitable for most situations, this blur level is evaluated on public datasets (Section \ref{evaluation}).

\subsubsection{Effect Evaluation and Methods Comparison}
\label{evaluation}

After the final schema of the privacy-preserving part and the blur level are decided, the effect of privacy-preserving methods should be evaluated using public datasets. The evaluation method is the same as that used in the Section \ref{blur}, by using the FaceNet model with threshold hold of cosine similarity = 0.5. The public datasets used here are UTKFace (In-the wild Faces) dataset, Real and Fake Face Detection dataset (RF), Celebahq dataset and LFW dataset. Details of the dataset could be found in Section \ref{datacollection}.

The experiment could be conducted in the following steps. Firstly, the ``blur without eyes" or ``mask without eyes" method is implemented on each image in the public datasets and these processed images are saved. Secondly, using the combined detector (MediaPipe + Dlib) to detect the faces in each image and extract them. Thirdly, comparing the original extracted face with the blurred or the masked face to calculate the recognition rate. The sketch map is depicted in \ref{fig:6_figture_1} and the result could be seen in \ref{tab:6_table_7}.


    \begin{figure*}[h]
    \centering
    \includegraphics[width=1\textwidth]{Doris_pic/evaluation.pdf}
    \caption{The sketch map of privacy preserving effect evaluation.}
    \label{fig:6_figture_1}
    \end{figure*} 

    \begin{table}[h]
    \centering
    \begin{tabular}{lllll}
    \toprule
     & \textbf{UTKFace} & \textbf{RF} & \textbf{Celebahq} & \textbf{LFW} \\ \midrule
    \textbf{Blur without Eyes} & 28.43\% & 0.63\% & 2.29\% & 0.71\%\\
    \textbf{Mask without Eyes} & 0.14\% & 0\% & 0\% & 0\%\\ 
    \bottomrule
    \end{tabular}
    \caption{The recognition rate of privacy preserving effect evaluation using public datasets.}
    \label{tab:6_table_7}
    \end{table}


As you can see in \ref{tab:6_table_7}, generally, the ``mask without eyes'' method performs really well with almost 0 recognition rates for all tested datasets. As for the ``blur without eyes'' method, it is good at the last three datasets, with a recognition rate lower than 5$\%$. However, for the UTKFace dataset, the result is not decent. This may be because that there are many young and elderly faces in this dataset who have more outstanding facial features such as big eyes for babies and deep wrinkles for the old man and then a bigger blur level is required. However, this is not a problem for our project since babies (under age 7) and elderly people (over age 60) are not the main populations that will take online education. Therefore, considering the effect of privacy-preserving and stability of the application, the ``mask without eyes" method is recommended.

In order to further compare these two privacy-preserving methods, the speed of the blurring process and mask process is tested on the local computer (i7-10710U, 16G RAM, Windows 10) for our self-made anomaly videos and the result could be seen in \ref{tab:6_table_8}.


    \begin{table}[h]
    \centering
    \begin{tabular}{ll}
    \toprule
    Method & FPS \\ \midrule
    \textbf{Blur Process} & 63 \\ 
    \textbf{Mask Process} & 28,852\\ 
    \bottomrule
    \end{tabular}
    \caption{The speed of privacy preserving methods on local computer.}
    \label{tab:6_table_8}
    \end{table}

It is obvious that the process of masking is much faster than that of blurring. This may be because that the blur method implemented in this project is Gaussian blur and the calculation of this method is heavy.

Although users' attitudes towards the blocking method are negative \citep{lr-25} when comparing with the blurring method, with comprehensive consideration, the ``mask without eyes" method is suggested in our project. This is not only because the effect of the ``mask without eyes" method is better and more stable, but also because the speed of mask method is much faster. Besides, the blur effect is negatively influenced by the resolution of the image which leads to instability of the blur method further.


\subsection{Anomaly Detection}
\subsubsection{Motion Detection}
\label{EE_motion}
\paragraph{Image Hashing Model}
There are some parameters in the image hashing model that we need to tune. For example, the hash size is originally set as 8, it will compress the image into an 8x8 greyscale image. However, a larger hash size will preserve more information compared to a smaller one. On the other hand, although the hash methods are introduced and discussed in the previous section, we will still conduct the experiment to justify which hash method is suitable for this task.

\subparagraph{Parameter Selection}
To select the most suitable hash method, we fix the hash size = 12 and use three hash methods we mentioned before to perform anomaly detection. The F1 score and running time are the major criteria for method selection.

    \begin{table}[h]
    \centering
    \begin{tabular}{lll}
    \toprule
    Hash Methods & F1 score & FPS\\ \midrule
    \textbf{dHash} & 0.8624 & 37\\ 
    aHash & 0.8426 & 37\\
    pHash & 0.8295 & 33\\
    \bottomrule
    \end{tabular}
    \caption{Performance summary for different hash methods with hash size = 12.}
    \label{tab:hash-comp}
    \end{table}

\ref{tab:hash-comp} shows that the dHash has the best performance for both criteria. The result is consistent with the experiment which is conducted by \citeauthor{dhash}. Therefore, we will use the dHash method to experiment with hash size. Hash size will be tested from 8 to 15. 

    \begin{figure*}[h]
    \centering
    \makebox[\textwidth][c]{
    \includegraphics[width=0.7\textwidth]{Pic/optimal_size.pdf}
    }
    \caption{Using F1 score to select the optimal hash size, the hash method is dHash.}
    \label{fig:hash_size}
    \end{figure*} 
    
\ref{fig:hash_size} illustrates that the highest F1 score can be obtained when hash size increases to 11. Higher or lower than this optimal hash size will deteriorate the model performance. Considering there is nearly no running time difference, thus we select the hash size = 11 as the optimal selection.

% \paragraph{Pose Detection Model}
% There is only one numerical parameter in this model, which is the threshold of shoulder difference in y-coordinate. We define the threshold as 0.05 in the first place, and we will use the grid search method to find the optimal threshold based on the test data. 

%     \begin{figure*}[h]
%     \centering
%     \makebox[\textwidth][c]{
%     \includegraphics[width=0.7\textwidth]{Pic/optimal_threshold.pdf}
%     }
%     \caption{Using F1 score to select the optimal shoulder landmark threshold.}
%     \label{fig:pose-threshold}
%     \end{figure*} 

% \ref{fig:pose-threshold} shows the highest accuracy can be obtained when the shoulder landmark threshold adjusts to 0.06. Therefore the optimal threshold for shoulder landmark will be set as 0.06 and the highest F1 score is 0.8680.
    

% \paragraph{Model Selection}
% Since we have selected the optimal parameters for both proposed models. We can now compare both models' performance in terms of F1 score and running time.

%     \begin{table}[h]
%     \centering
%     \begin{tabular}{lll}
%     \toprule
%     Hash Methods & F1 score & FPS\\ \midrule
%     \textbf{dHash model} & 0.8774 & 37\\ 
%     Pose detection model & 0.8680 & 9\\
%     \bottomrule
%     \end{tabular}
%     \caption{Model performance comparison table.}
%     \label{tab:model-comp}
%     \end{table}

% \ref{tab:model-comp} summarized the model performance evaluated on 5 video clips. In general, the dHash model outperforms the pose detection model for both criteria. dHash model has not only a higher F1 score but also significantly faster than the other. To be specific, hash model is capable of processing images up to 37 frames per second, which is 4 times faster than the pose detection model. Therefore, the dHash model will be selected as the final model for the motion anomaly detection task.

% \paragraph{Model Evaluation on Anonymized Videos}
% Since the proctoring system is designed to perform anomaly detection on the anonymized images such as blurred and masked images, it is essential to evaluate the model performance on the anonymized video clips. As we proposed two main anonymization functions, the image hashing model will be evaluated on blurred and masked images respectively.


%     \begin{table}[h]
%     \centering
%     \begin{tabular}{lll}
%     \toprule
%     anonymization & F1 score & FPS\\ \midrule
%     Blurring & 0.8709 & 31\\ 
%     Masking & 0.9010 & 35\\
%     \bottomrule
%     \end{tabular}
%     \caption{Model evaluation on masked and blurred testing frames.}
%     \label{tab:eva_ano}
%     \end{table}
    
% \ref{tab:eva_ano} shows that the dHash model maintains its performance on the anonymized data, its performance even better on the masking images. The running time of the model running on anonymized data maintains the same level as the original one. The difference may be caused by the Colab clouding environment. Considering the model performs well on both anonymization methods, we keep both blurring and masking functions in our system. For the best performance, we suggest using the masking method.

==> setup/macros.tex <==
%------------------------Custom Commands----------------------%

% = = = Latin Short-forms (ie, eg, etc, et al)
\usepackage{xspace}
\newcommand{\etal}{\textit{et al.}\xspace}
\newcommand{\etc}{\textit{etc.}\xspace}
\newcommand{\ie}{\textit{i.e.,}\xspace}
\newcommand{\eg}{\textit{e.g.,}\xspace}
\newcommand{\cf}{\textit{cf.}\xspace}
\newcommand{\supra}{\textit{Supra}\xspace}
\newcommand{\aka}{\textit{a.k.a.}\xspace}
% \mathchardef\-="2D
\mathchardef\mhyphen="2D


% correct bad hyphenation here
\hyphenation{op-tical net-works semi-conduc-tor}


% = = = Arrow -> (\lt)
\newcommand{\lt}{$\rightarrow$\xspace}
\newcommand{\framework}{\textsl{\mbox{PANDORA}}\xspace}

% = = = Keywords (kw)
\newcommand{\kw}[1]{\textsf{#1}}

% = = = Colored text (textblue)
\newcommand{\textblue}[1]{\textcolor{blue}{#1}}
\newcommand{\textred}[1]{\textcolor{red}{#1}}

% = = = Compact Lists (compactlist, compactlistn)
\newenvironment{compactlist}
  {\begin{itemize}
  \setlength{\itemsep}{0pt}
  \setlength{\parskip}{0pt}}
  {\end{itemize}}

\newenvironment{compactlistn}
  {\begin{enumerate}
  \setlength{\itemsep}{0pt}
  \setlength{\parskip}{0pt}}
  {\end{enumerate}}

\renewcommand{\labelitemi}{$\bullet$}

\newcommand{\pparagraph}[1]{\medskip \noindent \textbf{#1\ }}
\renewcommand{\paragraph}[1]{\medskip \noindent \textbf{#1.\ }}

\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}

\iffalse
\newtheorem{mydef}{Definition}
\newtheorem{theorem}{Theorem}
\newtheorem{proof}{Proof}
\newcommand*{\QEDA}{\hfill\ensuremath{\blacksquare}}
\fi

\newtheorem{definition}{Definition}
\newtheorem{theorem}{Theorem}


==> setup/packages.tex <==
\usepackage{wrapfig}
\usepackage{amsmath}
\usepackage{mathptmx}       % selects Times Roman as basic font
\usepackage{helvet}         % selects Helvetica as sans-serif font
\usepackage{courier}        % selects Courier as typewriter font
\usepackage{type1cm}        % activate if the above 3 fonts are
                            % not available on your system
\usepackage{makeidx}         % allows index generation
\usepackage{graphicx,subfigure}        % standard LaTeX graphics tool
                             % when including figure files
\usepackage{multicol}        % used for the two-column index
\usepackage[bottom]{footmisc}% places footnotes at page bottom
\usepackage{marvosym}
\usepackage{epstopdf}
\usepackage{epsfig}
\usepackage{algorithm}
\usepackage[noend]{algorithmic}
%\usepackage{subcaption}
\usepackage{amssymb}         % used for checkmark and times
\usepackage{wasysym}         % used for checkmark and times
%\usepackage{amsthm}
%\usepackage{dingbat}
\usepackage{diagbox}
\usepackage{subfigure}
\usepackage{cite}
\usepackage[hyphens]{url}
\usepackage{hyperref}
\usepackage{breakurl}
\usepackage{dsfont}
\usepackage{todonotes}
\usepackage{color}
%\usepackage{makecell}
\usepackage{caption}


==> title/title.tex <==
\begin{titlepage}
\newcommand{\HRule}{\rule{\linewidth}{0.5mm}}
\centering
\includegraphics[width=8cm]{title/logo.png}\\[1cm] 
\center 
% \quad\\[1.5cm]
\textsl{\Large The University of Sydney}\\[0.5cm] 
\textsl{\large Information Technology Capstone Project}\\[0.5cm] 
\makeatletter
\HRule \\[0.4cm]
{ \huge \bfseries \@title}\\[0.4cm] 
\HRule \\[1.5cm]
\begin{minipage}{0.4\textwidth}
\begin{flushleft} \large
\emph{Author:}\\
\@author 
\end{flushleft}
\end{minipage}
~
\begin{minipage}{0.4\textwidth}
\begin{flushright} \large
\emph{SID:} \\
\textup{440001665}\\
\textup{460255686}\\
\textup{490087398}\\
\textup{490606029}\\
\textup{490317158}\\
\end{flushright}
\end{minipage}\\[2cm]
\makeatother
{\large An Assignment submitted for the UoS:}\\[0.5cm]
{\large \emph{COMP5703/5707/5708}}\\[0.5cm]
{\large \today}\\[2cm] 
\vfill 
\end{titlepage}
